Deep Generative Sampling in the Dual Divergence Space: A Data-efficient & Interpretative Approach for Generative AI

Building on the remarkable achievements in generative sampling of natural images, we propose an innovative challenge, potentially overly ambitious, which involves generating samples of entire multivariate time series that resemble images. However, the statistical challenge lies in the small sample size, sometimes consisting of a few hundred subjects. This issue is especially problematic for deep generative models that follow the conventional approach of generating samples from a canonical distribution and then decoding or denoising them to match the true data distribution. In contrast, our method is grounded in information theory and aims to implicitly characterize the distribution of images, particularly the (global and local) dependency structure between pixels. We achieve this by empirically estimating its KL-divergence in the dual form with respect to the respective marginal distribution. This enables us to perform generative sampling directly in the optimized 1-D dual divergence space. Specifically, in the dual space, training samples representing the data distribution are embedded in the form of various clusters between two end points. In theory, any sample embedded between those two end points is in-distribution w.r.t. the data distribution. Our key idea for generating novel samples of images is to interpolate between the clusters via a walk as per gradients of the dual function w.r.t. the data dimensions. In addition to the data efficiency gained from direct sampling, we propose an algorithm that offers a significant reduction in sample complexity for estimating the divergence of the data distribution with respect to the marginal distribution. We provide strong theoretical guarantees along with an extensive empirical evaluation using many real-world datasets from diverse domains, establishing the superiority of our approach w.r.t. state-of-the-art deep learning methods.

==> math_commands.tex <==
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cTC}{{\mathcal{TC}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}
\newcommand{\newsetminus}{{\!-\!}}
\newcommand{\cVmA}{{\cV\newsetminus\cA}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cs}{s}
\newcommand{\cVms}{{\cV-\cs}}

\newcommand{\bE}{{\mathbb{E}}}

\newcommand{\kld}{{KL-D }}
% no space
\newcommand{\kldns}{{KL-D}}

\newcommand{\klp}{{KL-P* }}
\newcommand{\klpns}{{KL-P*}}

\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\resid}{\cR}

% \DeclareMathOperator{\MIF}{MI} 

\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\mhk}{\cM^h_k}

\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\prcref}[1]{Procedure~\ref{#1}}
\newcommand{\assmref}[1]{Assumption~\ref{#1}}
\newcommand{\crlref}[1]{Corollary~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\prpref}[1]{Proposition~\ref{#1}}
\newcommand{\cnjref}[1]{Conjecture~\ref{#1}}
\newcommand{\axmref}[1]{Axiom~\ref{#1}}
\newcommand{\lmaref}[1]{Lemma~\ref{#1}}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{procedure}[lemma]{Procedure}
\newtheorem{assumption}[lemma]{Assumption}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{conclusion}[lemma]{Conclusion}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{conjecture}[lemma]{Conjecture}
\newtheorem{axiom}[lemma]{Axiom}
\newtheorem{algo}[lemma]{Algorithm}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}


\DeclareMathOperator*{\argmax}{arg\,max}  % in your preamble
\DeclareMathOperator*{\argmin}{arg\,min}  % in your preamble 

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray} }
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation} }

\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*} }
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*} }


\newcommand{\R}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\Eh}{\hat{\mathbb{E}}}
\newcommand{\ph}{\hat{p}}
\newcommand{\Ph}{\hat{\mathbb{P}}}
\newcommand{\Th}{\hat{T}}
\newcommand{\fh}{\hat{f}}
\newcommand{\x}{\mathbf{x}}

%additions suggested by Sahil
\newcommand{\s}[1]{\textcolor{magenta}{#1}}


% \newcommand{\sa}[1]{ \textcolor{red}{\textbf{Sahil says to Anant}: #1}}

% %deletions suggested by Sahil
% \newcommand{\sd}[1]{\textcolor{orange}{#1}}

%additions suggested by Sahil
% \newcommand{\todo}[1]{\textcolor{blue}{Sahil's todo: #1}}

\newcommand{\todo}[1]{\textcolor{red}{#1}}

\newcommand{\rub}[1]{\textcolor{red}{From Rebuttal: #1}}

%additions suggested by Sahil
\newcommand{\ado}[1]{\textcolor{violet}{Anyone pls do: #1}}
    
%additions suggested by Mina
\newcommand{\mina}[1]{\textcolor{purple}{Mina says: #1}}

%additions suggested by Syamantak
\newcommand{\sdg}[1]{\textcolor{teal}{Syamantak: #1}}



==> other_tables_and_figs.tex <==
% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Lol lkl&Org.&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% \toprule
% % $\uparrow$ 
% NF&64$\pm$504&57$\pm$23&30$\pm$26&67$\pm$17&35$\pm$41&77$\pm$8\\
% \midrule
% % $\uparrow$ 
% DD & -0.02$\pm$0.17&-0.03$\pm$0.05&-0.14$\pm$0.27&-0.02$\pm$0.06&-0.02$\pm$0.16&-0.03$\pm$0.08\\
% \midrule
% % $\uparrow$ 
% KL-P*&-12$\pm$17&-14$\pm$4&-20$\pm$7&-52$\pm$31&-15$\pm$6&-11$\pm$4\\
% % \midrule
% % $\downarrow$ KL-D&0&14.2$\pm$0.02&-66.7$\pm$0.53&0.20$\pm$0.02&0.56$\pm$0.04&0.0$\pm$0.01\\
% \toprule
% \end{tabular}
% \caption{Sampling Evaluation for Finance.}
% \label{tab:finance_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% % \csizenine
% % \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log Lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% $\uparrow$ NF&-13$\pm$3&44$\pm$54&-7$\pm$5&17$\pm$3&41$\pm$3&79$\pm$159\\
% % \midrule
% % VAE&-0.69&-0.69&-0.77&-0.70&-0.69&-0.69\\
% \midrule
% $\uparrow$ DD&-0.69$\pm$1&-0.60$\pm$1&-0.66$\pm$1&-0.59$\pm$1&-0.58$\pm$1&-0.60$\pm$1\\
% \midrule
% KL-P*&-11$\pm$2&\\
% % \midrule
% % GAN&\\
% % \midrule
% % $\downarrow$ KL-D&&7.3$\pm$0.0&6.5$\pm$0.03&6.1$\pm$0.0&7.7$\pm$0.01&7.2$\pm$0.01\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for Synthetic~(d=20).}
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% NF&-21$\pm$2&82$\pm$17&-8$\pm$6&68$\pm$4&59$\pm$4&144$\pm$9\\
% % \midrule
% % VAE&-0.69&-0.69&-0.77&-0.70&-0.69&-0.69\\
% \midrule
% DD&-0.68$\pm$1.1&-0.60$\pm$1&-0.66$\pm$1&-0.58$\pm$1&-0.58$\pm$1&-0.60$\pm$1\\
% \midrule
% KL-P*&-17$\pm$3&-24$\pm$1&-24$\pm$1&-26$\pm$2&-24$\pm$1&-24$\pm$1\\
% % \midrule
% % GAN&\\
% % \midrule
% % $\downarrow$ KL-D&\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for Synthetic.}
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% % \csizenine
% % \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Eval. Metrics&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% $\uparrow$ NF&-72$\pm$2&275$\pm$52&-24$\pm$25&225$\pm$7&260$\pm$8&299$\pm$6\\
% % \midrule
% % VAE&-0.69&-0.69&-0.77&-0.70&-0.69&-0.69\\
% \midrule
% $\uparrow$ DD&-0.68$\pm$1.1&-0.60$\pm$1.1&-0.65$\pm$1.1&-0.58$\pm$1.1&-0.58$\pm$1.1&-0.60$\pm$1.1\\
% \midrule
% KL-P*&\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for Synthetic~(d=100).}
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% NF&46$\pm$26&174$\pm$31&263$\pm$69&137$\pm$6.4&148$\pm$5.4&361$\pm$139\\
% % \midrule
% % VAE&-0.69&-0.69&-0.77&-0.70&-0.69&-0.69\\
% \midrule
% DD&-0.59$\pm$1.1&-0.58$\pm$1.1&-0.59$\pm$1.1&-0.71$\pm$1.1&-0.73$\pm$1.1&-0.69$\pm$1.1\\
% \midrule
% KL-P*&1.6$\pm$2.9&-145$\pm$8&-0.09$\pm$4.1&-2.0$\pm$2.0&-198$\pm$9&-184$\pm$9\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for Neuroscience.}
% % 
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% NF&$\pm$&1551$\pm$583&1678$\pm$763&2197$\pm$239&1402$\pm$153&1969$\pm$136\\
% % \midrule
% % VAE&-0.69&-0.69&-0.77&-0.70&-0.69&-0.69\\
% \midrule
% DD&$\pm$&-0.03$\pm$0.05&-0.04$\pm$0.11&-0.02$\pm$0.05&-0.02$\pm$0.05&-0.03$\pm$0.10\\
% \midrule
% KL-P*&\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for NLP dataset.}
% % 
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% NF&-27$\pm$4&-15\pm$8&-24$\pm$8&-27$\pm$3&-18$\pm$4&34$\pm$5\\
% % \midrule
% % VAE&-0.69&-0.69&-0.77&-0.70&-0.69&-0.69\\
% \midrule
% DD&-0.9$\pm$1.3&-0.8$\pm$1.2&-1.0$\pm$1.4&-0.9$\pm$1.3&-0.6$\pm$1.0&-0.5$\pm$0.8\\
% \midrule
% KL-P*&-25$\pm$4&-92$\pm$0&-20$\pm$6&-45$\pm$23&-91$\pm$5&-27$\pm$11\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for Irish Wind dataset.}
% % 
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% NF&-26$\pm$47&-60\pm$39&-64$\pm$38&-33$\pm$27&-113$\pm$17&104$\pm$26\\
% \midrule
% DD&-0.5$\pm$0.7&-0.5$\pm$0.7&-0.8$\pm$1.1&-0.6$\pm$0.9&-0.6$\pm$0.9&-1.1$\pm$1.6\\
% \midrule
% KL-P*&-73$\pm$10&-161$\pm$0&-107$\pm$45&-161$\pm$0&-161$\pm$0&-80$\pm$20\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for Berkeley Lab Temperature dataset.}
% % 
% \label{tab:synthetic_sampling}
% \end{table*}

% \begin{table*}[tp!]
% \centering
% \csize
% \renewcommand{\tabcolsep}{2pt}
% \begin{tabular}{lllllll}
% \toprule
% Log lkl&Data&VAE&GAN&NF&DD&\textbf{KL-P*}\\
% % 
% \toprule
% NF&-214$\pm$67&194\pm$117&-128$\pm$96&-219$\pm$25&-249$\pm$22&190\pm$21\\
% \midrule
% DD$\pm$&-0.60\pm$0.94&-0.46$\pm$0.70&-0.65$\pm$0.97&-0.78$\pm$1.13&-0.58$\pm$0.92&-0.28$\pm$0.48\\
% \midrule
% KL-P*&-220$\pm$37&-181\pm$14&-161$\pm$14&-263$\pm$71&-270$\pm$60&-286$\pm$67\\
% % 
% \toprule
% % 
% \end{tabular}
% % 
% \caption{Sampling Evaluation for US Precipitation dataset.}
% % 
% \label{tab:synthetic_sampling}
% \end{table*}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


